Wave-Field Shaping in Cavities by Tunable Metasurfaces

Cavities, because they trap waves for long times due to their reflecting walls, are used in a vast number of scientific domains. Indeed, in these closed media and due to interferences, the free space continuum of solutions becomes a discrete set of stationary eigenmodes. These enhanced stationary fields are commonly used in fundamental physics to increase wave-matter interactions. The eigenmodes and associated eigenfrequencies of a cavity are imposed by its geometrical properties through the boundary conditions. In this paper, we show that one can control the wave fields created by point sources inside cavities by tailoring only the boundaries of the cavities. This is achieved through the use of a tunable reflecting metasurface, which is part of the frontiers of the cavity, and can switch its boundary conditions from Dirichlet to Neumann. Based on the use of arrays of subwavelength resonators, a mathematical modeling of the physical mechanism underlying the concept of tunable metasurfaces is provided.

==> layoutsetup.tex <==
%% Memoir layout setup

%% NOTE: You are strongly advised not to change any of them unless you
%% know what you are doing.  These settings strongly interact in the
%% final look of the document.

% Dependencies
\usepackage{ETHlogo}

% Turn extra space before chapter headings off.
\setlength{\beforechapskip}{0pt}

\nonzeroparskip
\parindent=0pt
\defaultlists

% Chapter style redefinition
\makeatletter

\if@twoside
  \pagestyle{Ruled}
  \copypagestyle{chapter}{Ruled}
\else
  \pagestyle{ruled}
  \copypagestyle{chapter}{ruled}
\fi
\makeoddhead{chapter}{}{}{}
\makeevenhead{chapter}{}{}{}
\makeheadrule{chapter}{\textwidth}{0pt}
\copypagestyle{abstract}{empty}

\makechapterstyle{bianchimod}{%
  \chapterstyle{default}
  \renewcommand*{\chapnamefont}{\normalfont\Large\sffamily}
  \renewcommand*{\chapnumfont}{\normalfont\Large\sffamily}
  \renewcommand*{\printchaptername}{%
    \chapnamefont\centering\@chapapp}
  \renewcommand*{\printchapternum}{\chapnumfont {\thechapter}}
  \renewcommand*{\chaptitlefont}{\normalfont\huge\sffamily}
  \renewcommand*{\printchaptertitle}[1]{%
    \hrule\vskip\onelineskip \centering \chaptitlefont\textbf{\vphantom{gyM}##1}\par}
  \renewcommand*{\afterchaptertitle}{\vskip\onelineskip \hrule\vskip
    \afterchapskip}
  \renewcommand*{\printchapternonum}{%
    \vphantom{\chapnumfont {9}}\afterchapternum}}

% Use the newly defined style
\chapterstyle{bianchimod}

\setsecheadstyle{\Large\bfseries\sffamily}
\setsubsecheadstyle{\large\bfseries\sffamily}
\setsubsubsecheadstyle{\bfseries\sffamily}
\setparaheadstyle{\normalsize\bfseries\sffamily}
\setsubparaheadstyle{\normalsize\itshape\sffamily}
\setsubparaindent{0pt}

% Set captions to a more separated style for clearness
\captionnamefont{\sffamily\bfseries\footnotesize}
\captiontitlefont{\sffamily\footnotesize}
\setlength{\intextsep}{16pt}
\setlength{\belowcaptionskip}{1pt}

% Set section and TOC numbering depth to subsection
\setsecnumdepth{subsection}
\settocdepth{subsection}

%% Titlepage adjustments
\pretitle{\vspace{0pt plus 0.7fill}\begin{center}\HUGE\sffamily\bfseries}
\posttitle{\end{center}\par}
\preauthor{\par\begin{center}\let\and\\\Large\sffamily}
\postauthor{\end{center}}
\predate{\par\begin{center}\Large\sffamily}
\postdate{\end{center}}

\def\@advisors{}
\newcommand{\advisors}[1]{\def\@advisors{#1}}
\def\@department{}
\newcommand{\department}[1]{\def\@department{#1}}
\def\@thesistype{}
\newcommand{\thesistype}[1]{\def\@thesistype{#1}}

\renewcommand{\maketitlehooka}{\noindent\ETHlogo[2in]}

\renewcommand{\maketitlehookb}{\vspace{1in}%
  \par\begin{center}\Large\sffamily\@thesistype\end{center}}

\renewcommand{\maketitlehookd}{%
  \vfill\par
  \begin{flushright}
    \sffamily
    \@advisors\par
    \@department, ETH Z\"urich
  \end{flushright}
}

\checkandfixthelayout

\setlength{\droptitle}{-48pt}

\makeatother

% This defines how theorems should look. Best leave as is.
\theoremstyle{plain}
\setlength\theorempostskipamount{0pt}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "thesis"
%%% End:


==> perturbation.tex <==
\chapter{Asymptotic Expansion to Perturbed Eigenvalues and Eigenfunctions}

Following the notations of previous chapter, we are going to derive the asymptotic expansion of eigenvalues and eigenfunctions to the perturbed Dirichlet problem. Let $\Omega\subset\mathbb{R}^2$ be a bounded set. $\partial\Omega=\partial\Omega_D\cup\partial\Omega_N$ is divided into two parts $\partial\Omega_D$ and $\partial\Omega_N$. Consider the following problem:

\begin{equation}\label{eq:problem}
	\left\{
		\begin{aligned}
			\Delta u^\epsilon + \mu^\epsilon u^\epsilon &= 0 \quad && \mathrm{in} && \mathbb{R}^2\backslash\partial\Omega, \\
			u^\epsilon &= 0 \quad && \mathrm{on} && \partial\Omega_D, \\
			\frac{\partial u^\epsilon}{\partial \nu} &= 0 \quad && \mathrm{on} && \partial\Omega_N,\\
		\end{aligned}
	\right.
\end{equation}
where $u^\epsilon$ satisfies outgoing radiation condition.

In this chapter we will still simplify $\partial\Omega_N$ as a small line segment which could be parametrized as
$$
\partial\Omega_N=\{(x,0):-\epsilon\leq x\leq\epsilon\}.
$$

Recall Dirichlet problem is defined to be
\begin{equation}\label{eq:dirichlet}
\left\{
\begin{aligned}
\Delta u + \mu u &= 0 \quad && \mathrm{in} && \Omega\,, \\
u &= 0 \quad && \mathrm{on} && \partial\Omega\,,\\
\end{aligned}
\right.
\end{equation}

and scattering Dirichlet problem is defined to be
\begin{equation}\label{eq:scatteringdirichlet}
\left\{
\begin{aligned}
\Delta u + \mu u &= 0 \quad && \mathrm{in} && \mathbb{R}^2\backslash\Omega\,, \\
u &= 0 \quad && \mathrm{on} && \partial\Omega\,,\\
\end{aligned}
\right.
\end{equation}
where $u$ satisfies outgoing radiation condition.

We will also use interior Dirichlet function $G_\Omega^\mu$ of \eqref{eq:dirichlet} as defined before(when $\mu$ is not an eigenvalue to \eqref{eq:dirichlet}) to be the unique solution of
\begin{equation}\label{eq:dirichletin}
\left\{
\begin{aligned}
(\Delta_x + \mu) G_\Omega^\mu(x,y) &= \delta_y(x) \quad && \mathrm{in}   && \Omega\,, \\
G_\Omega^\mu &= 0 \quad && \mathrm{on} && \partial\Omega\,,\\
\end{aligned}
\right.
\end{equation}

and exterior Dirichlet function $G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu$ of \eqref{eq:scatteringdirichlet}(when $\mu$ is not an eigenvalue to \eqref{eq:scatteringdirichlet}) to be the unique solution of
\begin{equation}\label{eq:dirichletex}
\left\{
\begin{aligned}
(\Delta_x + \mu)G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu(x,y) &= \delta_y(x) \quad && \mathrm{in} && \mathbb{R}^2\backslash\Omega, \\
G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu &= 0 \quad && \mathrm{on} && \partial\Omega,\\
\end{aligned}
\right.
\end{equation}
where $G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu$ satisfies outgoing radiation condition.

The existence and uniqueness of interior and exterior Dirichlet function is well-known. Furthermore, we know that the eigenvalues of interior Dirichlet problem \eqref{eq:dirichletin} and scattering poles of exterior Dirichlet problem \eqref{eq:dirichletex} are both set of discrete numbers. Suppose $\mu_0$ is an eigenvalue to interior Dirichlet problem with eigenfunction $u_{j0}$, there exists a small neighborhood V of $\mu_0$ depending on $\epsilon$, such that there is only one eigenvalue $\mu_\epsilon$ to \eqref{eq:problem} and no scattering pole in $V$. 

With similar proof of Lemma 2.1 of \cite{HaiHabib}, the following decomposition holds for $G_\Omega^\mu$ and $G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu$.
\begin{lemma}\label{lem:dirichletexpansion}
	Let $\mu_0$ be an eigenvalue to interior Dirichlet problem \eqref{eq:dirichletin} with eigenfunction $u_0$, and $V$ be one neighborhood of $\mu_0$ such that $\mu_0$ is the only eigenvalue of interior Dirichlet problem in $V$, and there is no scattering pole of exterior Dirichlet problem in $V$. Then for any $\mu\in V$, the interior Dirichlet function $G_\Omega^\mu$ satisfies
	\begin{equation}\label{eq:expansioninteriordirichlet}
	G_\Omega^\mu(x,y) = -\frac{1}{\pi}\ln|x-y| + \frac{u_0(x)u_0(y)}{\mu-\mu_0}+R_{\Omega,D}^{\mu,in}(x,y),\quad x \in \overline{\Omega}, y\in\partial\Omega, x\neq y, 
	\end{equation}
	and exterior Neumann function satisfies
	\begin{equation}\label{eq:expansionexteriordirichlet}
	G_{\mathbb{R}^2\backslash\Omega}^\mu(x,y) = -\frac{1}{\pi}\ln|x-y| + R_{\Omega,D}^{\mu,ex}(x,y), \quad x\in \mathbb{R}^2\backslash\Omega,y\in\partial\Omega, x\neq y,
	\end{equation}
	where $R_{\Omega,D}^{\mu,in}\in W^{3/2,2}(\overline\Omega)$ and $R_\Omega^{\mu,ex}\in W_{\mathrm{loc}}^{3/2,2}(\mathbb{R}^2\backslash\Omega)$. 
	\qed
\end{lemma}

\begin{remark}
	We make use of trace theorem to prove the regularity of $R_\Omega^{\mu,in}$ and $R_\Omega^{\mu,ex}$. One could refer to \cite{DZ1} for details.
\end{remark}


Suppose $u^\epsilon$ to be a solution of \eqref{eq:problem} with eigenvalue $\mu_0$, and $\varphi^\epsilon$ to be the normal derivative of $u^\epsilon$ on $\partial\Omega_D$. By Green's formula, we have
\begin{equation}\label{eq:equation1d}
\int_{\Omega}\Delta_y G_\Omega^\mu(x,y)u^\epsilon(y) - G_\Omega^\mu(x,y)\Delta_yu^\epsilon(y)\mathrm{d}y = \int_{\partial\Omega}\frac{\partial G_\Omega^\mu}{\partial\nu_y}(x,y)u^\epsilon(y) - G_\Omega^\mu(x,y)\frac{\partial u^\epsilon}{\partial\nu}(y)\mathrm{d}\sigma(y). 
\end{equation}
Notice that given $x\in\Omega$, the left part of \eqref{eq:equation1d} is $u^\epsilon(x)$, and right part is
$$
-\int_{\partial\Omega}u^\epsilon(y)\frac{\partial G_\Omega^\mu}{\partial\nu}(x,y)\mathrm{d}\sigma(y),
$$ 
therefore 
\begin{equation}\label{eq:equation2d}
u^\epsilon(x) =-\int_{\partial\Omega}u^\epsilon(y)\frac{\partial G_\Omega^\mu}{\partial\nu}(x,y)\mathrm{d}\sigma(y).
\end{equation}
With the same reasoning, given $x\in\mathbb{R}^2\backslash\Omega$, we could again apply Green's formula to exterior Neumann function $G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu$ and get
\begin{equation}
\begin{aligned}
&\int_{\Omega}\Delta_y N_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu(x,y)u^\epsilon(y) - N_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu(x,y)\Delta_yu^\epsilon(y)\mathrm{d}y \\
=& \int_{\partial\Omega}\frac{\partial N_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu}{\partial\nu_y^-}(x,y)u^\epsilon(y) - N_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu(x,y)\frac{\partial u^\epsilon}{\partial\nu^-_y}(y)\mathrm{d}\sigma(y),
\end{aligned}
\end{equation}
which implies that
\begin{equation}\label{eq:equation3d}
u^\epsilon(x) =  \int_{\partial\Omega}u^\epsilon(y)\frac{\partial G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu}{\partial\nu_y}(x,y)\mathrm{d}\sigma(y), \quad x\in\partial\Omega.
\end{equation}

Combine \eqref{eq:equation2d} and \eqref{eq:equation3d} we get
$$
\int_{-\epsilon}^{\epsilon}(G_{\mathbb{R}^2\backslash\overline{\Omega}}^{\sqrt{\mu}} + G_\Omega^{\sqrt{\mu}})(x,y)u^\epsilon(y)\mathrm{d}y = 0, \quad x\in\partial\Omega.
$$

If we define $\mathcal{A}^{ex}_\epsilon$ to be
$$
\mathcal{A}^{ex}_\epsilon(\mu)[\varphi](x):=\int_{-\epsilon}^{\epsilon}(G_{\mathbb{R}^2\backslash\overline{\Omega}}^{\sqrt{\mu}} + G_\Omega^{\sqrt{\mu}})(x,y)u^\epsilon(y)\mathrm{d}y,\quad x\in\partial\Omega,
$$	
any eigenvalue $\mu^\epsilon$ of \eqref{eq:problem} is also a characteristic value of $\mathcal{A}^{ex}_\epsilon$. Therefore we only need to examine the property of $\mathcal{A}^{ex}_\epsilon$, which could be done by decomposing the operator into several parts.

Define
$$
\mathcal{K}_\epsilon[\varphi](x):=(\varphi,u_{j0})u_{j0} = (\int_{-\epsilon}^{\epsilon}u_{j0}(y)\varphi(y)\mathrm{d}y)u_{j0}(x)
$$ and 
$$
\mathcal{R}_\epsilon[\varphi](x) := \int_{-\epsilon}^\epsilon R(\mu,x,y)\varphi(y)\mathrm{d}y := \int_{-\epsilon}^\epsilon (R_{\Omega,D}^{\mu,in}+R_{\Omega,D}^{\mu,ex})(x,y)\varphi(y)\mathrm{d}y,
$$
where $(\mu,x,y)\mapsto R(\mu,x,y)$ is holomorphic in $\mu$ and of class $\mathcal{C}^{1,\alpha}$ in $x$ and $y$, for $0<\alpha<1$.

The following lemmas will be of useful in later proof.

\begin{lemma}\label{lem:lem52d}(Lemma 5.2 of \cite{LPTSA})
	For all $0<\epsilon<2$, the integral operator $\mathcal{L}_\epsilon:\mathcal{X}^\epsilon\mapsto\mathcal{Y}^\epsilon$ is invertible.
\end{lemma}

\begin{lemma}\label{lem:lem54d}(Lemma 5.4 of \cite{LPTSA})
	Let $\mathcal{R}_\epsilon$ be the integral operator defined from $\mathcal{X}^\epsilon$ into $\mathcal{Y}^\epsilon$ by 
	$$
	\mathcal{R}_\epsilon[\varphi](x) = \int_{-\epsilon}^\epsilon R(x,y)\varphi(y)\mathrm{d}y
	$$
	with $R(x,y)$ of class $\mathcal{C}^{1,\alpha}$ in $x$ and $y$, for $0<\alpha<1$. There exists a positive constant $C$, independent of $\epsilon$, such that
	\begin{equation}
	\|\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon\|_{\mathcal{L}(\mathcal{X}^\epsilon,\mathcal{X}^\epsilon)}\leq\frac{C}{\ln\epsilon},
	\end{equation}
	where
	$$
	\|\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon\|_{\mathcal{L}(\mathcal{X}^\epsilon,\mathcal{X}^\epsilon)} = \sup\limits_{\varphi\in\mathcal{X}^\epsilon,\|\varphi\|_{\mathcal{X}^\epsilon}=1}\|\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon[\varphi]\|_{\mathcal{X}^\epsilon}.
	$$
\end{lemma}

With Lemma \ref{lem:lem54d}, Lemma \ref{lem:lem52d} and pole-pencil decomposition in Lemma \ref{lem:dirichletexpansion}, we have the following important decomposition theorem for $\mathcal{A}_\epsilon^{ex}$:
\begin{theorem}\label{thm:polepencildirichlet}
	The following pole-pencil decomposition of $\mathcal{A}_\epsilon(\mu):\mathcal{X}^\epsilon\rightarrow\mathcal{Y}^\epsilon$ holds for any $\mu\in V\backslash\{\mu_0\}$:
	\begin{equation}\label{eq:polepencildirichlet}
	\mathcal{A}^{ex}_\epsilon(\mu) = -\frac{2}{\pi}\mathcal{L}_\epsilon + \frac{\mathcal{K}_\epsilon}{\mu_0-\mu} + \mathcal{R}_\epsilon(\mu).
	\end{equation}
\end{theorem}
\begin{proof}
	From Lemma 5.1 of \cite{LPTSA}, we learn that
	$$
	\mathcal{A}_\epsilon(\mu)[\varphi](x):=\int_{-\epsilon}^{\epsilon} G_\Omega^{\sqrt{\mu}}(x,y)\varphi(y)\mathrm{d}y,
	$$
	has the decomposition
	$$
	\mathcal{A}_\epsilon(\mu) = -\frac{1}{\pi}\mathcal{L}_\epsilon + \frac{\mathcal{K}_\epsilon}{\mu_0-\mu} + \mathcal{R}^0_\epsilon(\mu),
	$$
	where $\mathcal{R}_\epsilon^0(\mu)$ is also holomorphic with respect to $\mu$.
	so
	\begin{align*}
	\mathcal{A}_\epsilon^{ex}(\mu)[\varphi] &= \mathcal{A}_\epsilon(\mu)[\varphi] + \int_{-\epsilon}^{\epsilon}G_{\mathbb{R}^2\backslash\overline{\Omega}}^{\sqrt{\mu}}(x,y)\varphi(y)\mathrm{d}y \\
	&= -\frac{2}{\pi}\mathcal{L}_\epsilon[\varphi] + \frac{\mathcal{K}_\epsilon[\varphi]}{\mu_0-\mu} + (\mathcal{R}_\epsilon^0(\mu)[\varphi] + \int_{-\epsilon}^\epsilon r(x,y,\mu)\varphi(y)\mathrm{d}y).
	\end{align*}
	The final result follows if we define $\mathcal{R}_\epsilon(\mu)[\varphi]:=\mathcal{R}_\epsilon^0(\mu)[\varphi] + \int_{-\epsilon}^\epsilon r(x,y,\mu)\varphi(y)\mathrm{d}y$.
\end{proof}

With help of theorem \ref{thm:polepencildirichlet} and generalization of Steinberg theorem(Theorem 1.16 in \cite{LPTSA}), we could prove the following two important properties of characteristic value of $\mathcal{A}_\epsilon^{ex}$:

\begin{lemma}\label{lem:discretedirichlet}
	The set of characteristic values of $\mu\mapsto\mathcal{A}_\epsilon^{ex}(\mu)$ is discrete.
\end{lemma}
\begin{proof}
	Let $V$ be the same neighborhood of $\mu_0$ chosen in Lemma \ref{lem:dirichletexpansion}. We first prove the conclusion in $V$. Notice that $\mathcal{L}_\epsilon:\mathcal{X}^\epsilon\rightarrow\mathcal{Y}^\epsilon$ is invertible and $\|\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon\|_{\mathcal{L}(\mathcal{X}^\epsilon,\mathcal{X}^\epsilon)}\rightarrow 0$ as $\epsilon\rightarrow 0$. Therefore $-(2/\pi)\mathcal{L}_\epsilon + \mathcal{R}_\epsilon:\mathcal{X}^\epsilon\rightarrow\mathcal{Y}^\epsilon$ is invertible given $\epsilon$ small enough. We can then conclude from the decomposition \eqref{eq:polepencildirichlet} that $\mathcal{A}_\epsilon^{ex}$ is finitely meromorphic and of Fredholm type. In fact, $\frac{\mathcal{K}_\epsilon}{\mu_0-\mu}$ implies the pole of $\mathcal{A}_\epsilon^{ex}$ is order 1. Moreover, $\mathcal{A}_\epsilon^{ex}-\frac{\mathcal{K}_\epsilon}{\mu_0-\mu}$ is Fredholm because $\mathcal{L}_\epsilon:\mathcal{X}^\epsilon\rightarrow\mathcal{Y}^\epsilon_0$ is invertible and $\mathcal{R}_\epsilon$ is compact. Since $\mathcal{K}_\epsilon$ is finite dimension, there exists $\mu^*\in V$ such that $\mathcal{A}_\epsilon(\mu^*)$ is invertible. Therefore, the generalization of the Steinberg theorem gives the discreteness of set of characteristic values of $\mathcal{A}_\epsilon^{ex}$ in $V$. With the same method we could prove the result in each neighborhood $V_j$ of $\mu_j$, where $\mu_j$ is any eigenvalue to interior Dirichlet problem \eqref{eq:dirichlet}, and in $\mathbb{R}^2\backslash\bigcup_j V_j$.
\end{proof}

\begin{lemma}\label{lem:onechardirichlet}
	The operator-valued function $\mathcal{A}_\epsilon(\mu)$ has exactly one characteristic value in $V$, where $V$ is the same as Lemma \ref{lem:dirichletexpansion}.
\end{lemma}
\begin{proof}
	First we define the principal part of $\mathcal{A}_\epsilon^{ex}$:
	$$
		\mathcal{N}_\epsilon:=-\frac{2}{\pi}\mathcal{L}_\epsilon + \frac{\mathcal{K}_\epsilon}{\mu_0-\mu}.
	$$
	Now we would like to find the characteristic value of $\mathcal{N}_\epsilon$ in $V$. Suppose we have complex number $\tilde{\mu}$ and function $\tilde{\varphi}$ satisfying $\mathcal{N}_\epsilon(\tilde{\mu})[\tilde{\varphi}]=0$ on $(-\epsilon,\epsilon)$. $\tilde{\mu}$ and $\tilde{\varphi}$ then satisfies
	$$
		\frac{2}{\pi}\mathcal{L}_\epsilon[\tilde{\varphi}] + \frac{(\tilde{\varphi},u_{j0})}{\tilde{\mu}-\mu_0}u_{j0} = 0,
	$$
	which is
	$$
		\frac{2}{\pi}\tilde{\varphi} + \frac{(\tilde{\varphi},u_{j0})}{\tilde{\mu}-\mu_0}\mathcal{L}_\epsilon^{-1}[u_{j0}] = 0.
	$$
	Taking $L^2$ inner product on $(-\epsilon,\epsilon)$ on both side with $u_{j0}$, we have
	$$
		(\tilde{\varphi},u_{j0})\left(\frac{2}{\pi} + \frac{(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})}{\tilde{\mu}-\mu_0}\right) = 0,
	$$
	which means
	$$
		\tilde{\mu} = \mu_0 - \frac{\pi}{2}(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0}).
	$$
	Since $|(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})|\rightarrow 0$ as $\epsilon\rightarrow 0$, by choosing a sufficiently small $\epsilon$ we can always ensure that $\tilde{\mu}$ lies in $V$. The corresponding root function is 
	$$
		\tilde{\varphi} = \frac{\mathcal{L}_\epsilon^{-1}[u_{j0}]}{(\mathcal{L}_\epsilon^{-1}[u_{j0}], u_{j0})},
	$$
	if without loss of generality we assume $(\tilde{\varphi}, u_{j0}) =1$.
	Now we want to study the multiplicity of $\tilde{\mu}$ as a characteristic value of $\mathcal{N}_\epsilon$ in $V$. Suppose $\varphi$ and $f$ satisfies $\mathcal{N}_\epsilon(\mu)[\varphi]=f$, then
	$$
		-\frac{2}{\pi}\varphi + \frac{(\varphi,u_{j0})\mathcal{L}_\epsilon^{-1}[u_{j0}]}{\mu_0-\mu} = \mathcal{L}_\epsilon^{-1}[f].
	$$
	Therefore
	$$
		(\varphi,u_{j0})\left[-\frac{2}{\pi} + \frac{(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})}{\mu_0-\mu}\right] = (\mathcal{L}_\epsilon^{-1}[f],u_{j0}),
	$$
	which implies 
	$$
		(\varphi,u_{j0}) = \frac{\pi(\mu_0-\mu)}{2(\mu-\tilde{\mu})}(\mathcal{L}_\epsilon^{-1}[f],u_{j0}).
	$$
	We then have
	$$
	\varphi = -\frac{\pi}{2}\mathcal{L}_\epsilon^{-1}[f] + \frac{\pi^2}{4}\frac{(\mathcal{L}_\epsilon^{-1}[f],u_{j0})}{\mu-\tilde{\mu}}\mathcal{L}^{-1}_\epsilon[u_{j0}].
	$$
	Hence we could conclude that $\tilde{\mu}$ is the only characteristic value of $\mathcal{N}_\epsilon$ in $V$ and it is of order one.
	
	Now we examine the multiplicity of $\mathcal{A}_\epsilon^{ex}$ in $V$. It is obvious that $\mathcal{N}_\epsilon$ is normal and 
	$$
		\lim\limits_{\epsilon\rightarrow 0}\|\mathcal{N}_\epsilon^{-1}(\mu)\mathcal{R}_\epsilon(\mu)\|_{\mathcal{L}(\mathcal{X}^\epsilon,\mathcal{X}^\epsilon)} = 0, \quad\forall\mu\in\partial V.
	$$
	By generalized Rouch\'e theorem, $\mathcal{A}_\epsilon^{ex}$ has exactly one characteristic value $\mu^\epsilon$ in $V$.
\end{proof}

In view of Lemma \ref{lem:discretedirichlet}, Lemma \ref{lem:onechardirichlet} and Theorem \ref{thm:polepencildirichlet}, we could finally prove the main result of this chapter.
\begin{theorem}
	The operator-valued function $\mathcal{A}^{ex}_\epsilon(\mu)$ has exactly one characteristic value $\mu^\epsilon$ in $V$. Moreover, the following approximation of $\mu^\epsilon$ and $\varphi_\epsilon$ holds:
	\begin{equation}\label{eq:eigasymdirichlet}
	\mu^\epsilon=\mu_0-\pi(\mathcal{L}_\epsilon^{-1}[u_{j_0}],u_{j_0}) + \pi^2(\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon(\mu_0)\mathcal{L}_\epsilon^{-1}[u_{j_0}],u_{j_0}) + O(|\ln\epsilon|^{-2}) + O(|\ln\epsilon|^{-2}),
	\end{equation}
	\begin{equation}\label{eq:solasymdirichlet}
	\varphi_\epsilon = \frac{\mathcal{L}_\epsilon^{-1}[u_{j0}]}{(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})} + O(|\ln\epsilon|^{-1}).
	\end{equation}
\end{theorem}
\begin{proof}
	
	Denote $\varphi_\epsilon$ as the corresponding root function of $\mathcal{A}^{ex}_\epsilon(\mu)$. Therefore we have
	\begin{equation}
	\frac{1}{\pi}\mathcal{L}_\epsilon[\varphi_\epsilon] + \frac{(\varphi_\epsilon,u_{j0})}{\mu_\epsilon-\mu_0}u_{j0} - \mathcal{R}_\epsilon[\varphi_\epsilon]=0.
	\end{equation}
	By Lemma 5.2 in \cite{LPTSA}, $\mathcal{L}_\epsilon$ is invertible. Therefore
	\begin{equation}\label{eq:varphi1d}
	\frac{1}{\pi}\varphi_\epsilon + \frac{(\varphi_\epsilon,u_{j0})}{\mu_\epsilon-\mu_0}\mathcal{L}_\epsilon^{-1}[u_{j0}] - \mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon[\varphi_\epsilon]=0.
	\end{equation}
	Taking inner product against $u_{j0}$ on both side, we get
	\begin{equation}
	\frac{1}{\pi} + \frac{(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})}{\mu_\epsilon-\mu_0} - (\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon[\varphi_\epsilon],u_{j0}) = 0,
	\end{equation}
	that is,
	\begin{equation}\label{eq:equation4d}
	\mu_\epsilon - \mu_0 + \pi(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})-\pi(\mu_\epsilon-\mu_0)(\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon[\varphi_\epsilon],u_{j0}) =0.
	\end{equation}
	Since $\|\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon\|_{\mathcal{L}(\mathcal{X}^\epsilon,\mathcal{X}^\epsilon)}\leq\frac{C}{\ln\epsilon}$, and $\mathcal{L}_\epsilon^{-1}[u_{j0}] = O(|\ln\epsilon|^{-1})$, we know $\mu_\epsilon - \mu_0 = O(|\ln\epsilon|^{-1})$. Plug it back into \eqref{eq:equation4d}, we have that
	\begin{equation}\label{eq:equation5d}
	\mu_\epsilon - \mu_0 = -\pi(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0}) + O(|\ln\epsilon|^{-2}).
	\end{equation}
	Meanwhile, from \eqref{eq:varphi1d} it follows that
	\begin{equation}\label{eq:varphi2d}
	\varphi_\epsilon = -\frac{\pi}{\mu_\epsilon-\mu_0}\mathcal{L}_\epsilon^{-1}[u_{j0}]+\pi \mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon[\varphi_\epsilon]
	\end{equation}
	Combining \eqref{eq:equation4d} and \eqref{eq:varphi2d} implies
	\begin{equation}\label{eq:dirichleteigexpansion}
	\mu_\epsilon = \mu_0 -\pi(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0}) + \pi^2(\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0}) + O(|\ln\epsilon|^{-2}).
	\end{equation}
	Combining \eqref{eq:equation5d} and \eqref{eq:varphi1d} leads to
	\begin{equation}\label{eq:dirichletsolexpansion}
	\varphi_\epsilon = \frac{\mathcal{L}_\epsilon^{-1}[u_{j0}]}{(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})} + O(|\ln\epsilon|^{-1}).
	\end{equation}
\end{proof}



==> perturbation2.tex <==
\chapter{Asymptotic Expansion to Perturbed Eigenvalues, Eigenfunctions and Numerical Implementation}

\section{Asymptotic Expansion to Perturbed Eigenvalues and Eigenfunctions}
Following the notations of previous chapter, we are going to derive the asymptotic expansion of eigenvalues and eigenfunctions to the perturbed Dirichlet problem. Let $\Omega\subset\mathbb{R}^2$ be a bounded set. $\partial\Omega=\partial\Omega_D\cup\partial\Omega_N$ is divided into two parts $\partial\Omega_D$ and $\partial\Omega_N$. Consider the following problem:

\begin{equation}\label{eq:problem}
	\left\{
		\begin{aligned}
			\Delta u^\epsilon + \mu^\epsilon u^\epsilon &= 0 \quad && \mathrm{in} && \mathbb{R}^2\backslash\partial\Omega, \\
			u^\epsilon &= 0 \quad && \mathrm{on} && \partial\Omega_D, \\
			\frac{\partial u^\epsilon}{\partial \nu} &= 0 \quad && \mathrm{on} && \partial\Omega_N,\\
		\end{aligned}
	\right.
\end{equation}
where $u^\epsilon$ satisfies outgoing radiation condition.

In this chapter we will still simplify $\partial\Omega_N$ as a small line segment which could be parametrized as
$$
\partial\Omega_N=\{(x,0):-\epsilon\leq x\leq\epsilon\}.
$$

Recall Dirichlet problem is defined to be
\begin{equation}\label{eq:dirichlet}
\left\{
\begin{aligned}
\Delta u + \mu u &= 0 \quad && \mathrm{in} && \Omega\,, \\
u &= 0 \quad && \mathrm{on} && \partial\Omega\,,\\
\end{aligned}
\right.
\end{equation}

and scattering Dirichlet problem is defined to be
\begin{equation}\label{eq:scatteringdirichlet}
\left\{
\begin{aligned}
\Delta u + \mu u &= 0 \quad && \mathrm{in} && \mathbb{R}^2\backslash\Omega\,, \\
u &= 0 \quad && \mathrm{on} && \partial\Omega\,,\\
\end{aligned}
\right.
\end{equation}
where $u$ satisfies outgoing radiation condition.

We will also use interior Dirichlet function $G_\Omega^\mu$ of \eqref{eq:dirichlet} as defined before(when $\mu$ is not an eigenvalue to \eqref{eq:dirichlet}) to be the unique solution of
\begin{equation}\label{eq:dirichletin}
\left\{
\begin{aligned}
(\Delta_x + \mu) G_\Omega^\mu(x,y) &= \delta_y(x) \quad && \mathrm{in}   && \Omega\,, \\
G_\Omega^\mu &= 0 \quad && \mathrm{on} && \partial\Omega\,,\\
\end{aligned}
\right.
\end{equation}

and exterior Dirichlet function $G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu$ of \eqref{eq:scatteringdirichlet}(when $\mu$ is not an eigenvalue to \eqref{eq:scatteringdirichlet}) to be the unique solution of
\begin{equation}\label{eq:dirichletex}
\left\{
\begin{aligned}
(\Delta_x + \mu)G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu(x,y) &= \delta_y(x) \quad && \mathrm{in} && \mathbb{R}^2\backslash\Omega, \\
G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu &= 0 \quad && \mathrm{on} && \partial\Omega,\\
\end{aligned}
\right.
\end{equation}
where $G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu$ satisfies outgoing radiation condition.

The existence and uniqueness of interior and exterior Dirichlet function is well-known. Furthermore, we know that the eigenvalues of interior Dirichlet problem \eqref{eq:dirichletin} and scattering poles of exterior Dirichlet problem \eqref{eq:dirichletex} are both set of discrete numbers. Suppose $\mu_0$ is an eigenvalue to interior Dirichlet problem with eigenfunction $u_{j0}$, there exists a small neighborhood V of $\mu_0$ depending on $\epsilon$, such that there is only one eigenvalue $\mu_\epsilon$ to \eqref{eq:problem} and no scattering pole in $V$. 

With similar proof of Lemma 2.1 of \cite{HaiHabib}, the following decomposition holds for $G_\Omega^\mu$ and $G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu$.
\begin{lemma}\label{lem:dirichletexpansion}
	Let $\mu_0$ be an eigenvalue to interior Dirichlet problem \eqref{eq:dirichletin} with eigenfunction $u_0$, and $V$ be one neighborhood of $\mu_0$ such that $\mu_0$ is the only eigenvalue of interior Dirichlet problem in $V$, and there is no scattering pole of exterior Dirichlet problem in $V$. Then for any $\mu\in V$, the interior Dirichlet function $G_\Omega^\mu$ satisfies
	\begin{equation}\label{eq:expansioninteriordirichlet}
	G_\Omega^\mu(x,y) = -\frac{1}{\pi}\ln|x-y| + \frac{u_0(x)u_0(y)}{\mu-\mu_0}+R_{\Omega,D}^{\mu,in}(x,y),\quad x \in \overline{\Omega}, y\in\partial\Omega, x\neq y, 
	\end{equation}
	and exterior Neumann function satisfies
	\begin{equation}\label{eq:expansionexteriordirichlet}
	G_{\mathbb{R}^2\backslash\Omega}^\mu(x,y) = -\frac{1}{\pi}\ln|x-y| + R_{\Omega,D}^{\mu,ex}(x,y), \quad x\in \mathbb{R}^2\backslash\Omega,y\in\partial\Omega, x\neq y,
	\end{equation}
	where $R_{\Omega,D}^{\mu,in}\in W^{3/2,2}(\overline\Omega)$ and $R_\Omega^{\mu,ex}\in W_{\mathrm{loc}}^{3/2,2}(\mathbb{R}^2\backslash\Omega)$. 
	\qed
\end{lemma}

\begin{remark}
	We make use of trace theorem to prove the regularity of $R_\Omega^{\mu,in}$ and $R_\Omega^{\mu,ex}$. One could refer to \cite{DZ1} for details.
\end{remark}


Suppose $u^\epsilon$ to be a solution of \eqref{eq:problem} with eigenvalue $\mu_0$, and $\varphi^\epsilon$ to be the normal derivative of $u^\epsilon$ on $\partial\Omega_D$. By Green's formula, we have
\begin{equation}\label{eq:equation1d}
\int_{\Omega}\Delta_y G_\Omega^\mu(x,y)u^\epsilon(y) - G_\Omega^\mu(x,y)\Delta_yu^\epsilon(y)\mathrm{d}y = \int_{\partial\Omega}\frac{\partial G_\Omega^\mu}{\partial\nu_y}(x,y)u^\epsilon(y) - G_\Omega^\mu(x,y)\frac{\partial u^\epsilon}{\partial\nu}(y)\mathrm{d}\sigma(y). 
\end{equation}
Notice that given $x\in\Omega$, the left part of \eqref{eq:equation1d} is $u^\epsilon(x)$, and right part is
$$
-\int_{\partial\Omega}u^\epsilon(y)\frac{\partial G_\Omega^\mu}{\partial\nu}(x,y)\mathrm{d}\sigma(y),
$$ 
therefore 
\begin{equation}\label{eq:equation2d}
u^\epsilon(x) =-\int_{\partial\Omega}u^\epsilon(y)\frac{\partial G_\Omega^\mu}{\partial\nu}(x,y)\mathrm{d}\sigma(y).
\end{equation}
With the same reasoning, given $x\in\mathbb{R}^2\backslash\Omega$, we could again apply Green's formula to exterior Neumann function $G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu$ and get
\begin{equation}
\begin{aligned}
&\int_{\Omega}\Delta_y N_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu(x,y)u^\epsilon(y) - N_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu(x,y)\Delta_yu^\epsilon(y)\mathrm{d}y \\
=& \int_{\partial\Omega}\frac{\partial N_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu}{\partial\nu_y^-}(x,y)u^\epsilon(y) - N_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu(x,y)\frac{\partial u^\epsilon}{\partial\nu^-_y}(y)\mathrm{d}\sigma(y),
\end{aligned}
\end{equation}
which implies that
\begin{equation}\label{eq:equation3d}
u^\epsilon(x) =  \int_{\partial\Omega}u^\epsilon(y)\frac{\partial G_{\mathbb{R}^2\backslash\overline{\Omega}}^\mu}{\partial\nu_y}(x,y)\mathrm{d}\sigma(y), \quad x\in\partial\Omega.
\end{equation}

Combine \eqref{eq:equation2d} and \eqref{eq:equation3d} we get
$$
\int_{-\epsilon}^{\epsilon}(G_{\mathbb{R}^2\backslash\overline{\Omega}}^{\sqrt{\mu}} + G_\Omega^{\sqrt{\mu}})(x,y)u^\epsilon(y)\mathrm{d}y = 0, \quad x\in\partial\Omega.
$$

If we define $\mathcal{A}^{ex}_\epsilon$ to be
$$
\mathcal{A}^{ex}_\epsilon(\mu)[\varphi](x):=\int_{-\epsilon}^{\epsilon}(G_{\mathbb{R}^2\backslash\overline{\Omega}}^{\sqrt{\mu}} + G_\Omega^{\sqrt{\mu}})(x,y)u^\epsilon(y)\mathrm{d}y,\quad x\in\partial\Omega,
$$	
any eigenvalue $\mu^\epsilon$ of \eqref{eq:problem} is also a characteristic value of $\mathcal{A}^{ex}_\epsilon$. Therefore we only need to examine the property of $\mathcal{A}^{ex}_\epsilon$, which could be done by decomposing the operator into several parts.

Define
$$
\mathcal{K}_\epsilon[\varphi](x):=(\varphi,u_{j0})u_{j0} = (\int_{-\epsilon}^{\epsilon}u_{j0}(y)\varphi(y)\mathrm{d}y)u_{j0}(x)
$$ and 
$$
\mathcal{R}_\epsilon[\varphi](x) := \int_{-\epsilon}^\epsilon R(\mu,x,y)\varphi(y)\mathrm{d}y := \int_{-\epsilon}^\epsilon (R_{\Omega,D}^{\mu,in}+R_{\Omega,D}^{\mu,ex})(x,y)\varphi(y)\mathrm{d}y,
$$
where $(\mu,x,y)\mapsto R(\mu,x,y)$ is holomorphic in $\mu$ and of class $\mathcal{C}^{1,\alpha}$ in $x$ and $y$, for $0<\alpha<1$.

The following lemmas will be of useful in later proof.

\begin{lemma}\label{lem:lem52d}(Lemma 5.2 of \cite{LPTSA})
	For all $0<\epsilon<2$, the integral operator $\mathcal{L}_\epsilon:\mathcal{X}^\epsilon\mapsto\mathcal{Y}^\epsilon$ is invertible.
\end{lemma}

\begin{lemma}\label{lem:lem54d}(Lemma 5.4 of \cite{LPTSA})
	Let $\mathcal{R}_\epsilon$ be the integral operator defined from $\mathcal{X}^\epsilon$ into $\mathcal{Y}^\epsilon$ by 
	$$
	\mathcal{R}_\epsilon[\varphi](x) = \int_{-\epsilon}^\epsilon R(x,y)\varphi(y)\mathrm{d}y
	$$
	with $R(x,y)$ of class $\mathcal{C}^{1,\alpha}$ in $x$ and $y$, for $0<\alpha<1$. There exists a positive constant $C$, independent of $\epsilon$, such that
	\begin{equation}
	\|\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon\|_{\mathcal{L}(\mathcal{X}^\epsilon,\mathcal{X}^\epsilon)}\leq\frac{C}{\ln\epsilon},
	\end{equation}
	where
	$$
	\|\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon\|_{\mathcal{L}(\mathcal{X}^\epsilon,\mathcal{X}^\epsilon)} = \sup\limits_{\varphi\in\mathcal{X}^\epsilon,\|\varphi\|_{\mathcal{X}^\epsilon}=1}\|\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon[\varphi]\|_{\mathcal{X}^\epsilon}.
	$$
\end{lemma}

With Lemma \ref{lem:lem54d}, Lemma \ref{lem:lem52d} and pole-pencil decomposition in Lemma \ref{lem:dirichletexpansion}, we have the following important decomposition theorem for $\mathcal{A}_\epsilon^{ex}$:
\begin{theorem}\label{thm:polepencildirichlet}
	The following pole-pencil decomposition of $\mathcal{A}_\epsilon(\mu):\mathcal{X}^\epsilon\rightarrow\mathcal{Y}^\epsilon$ holds for any $\mu\in V\backslash\{\mu_0\}$:
	\begin{equation}\label{eq:polepencildirichlet}
	\mathcal{A}^{ex}_\epsilon(\mu) = -\frac{2}{\pi}\mathcal{L}_\epsilon + \frac{\mathcal{K}_\epsilon}{\mu_0-\mu} + \mathcal{R}_\epsilon(\mu).
	\end{equation}
\end{theorem}
\begin{proof}
	From Lemma 5.1 of \cite{LPTSA}, we learn that
	$$
	\mathcal{A}_\epsilon(\mu)[\varphi](x):=\int_{-\epsilon}^{\epsilon} G_\Omega^{\sqrt{\mu}}(x,y)\varphi(y)\mathrm{d}y,
	$$
	has the decomposition
	$$
	\mathcal{A}_\epsilon(\mu) = -\frac{1}{\pi}\mathcal{L}_\epsilon + \frac{\mathcal{K}_\epsilon}{\mu_0-\mu} + \mathcal{R}^0_\epsilon(\mu),
	$$
	where $\mathcal{R}_\epsilon^0(\mu)$ is also holomorphic with respect to $\mu$.
	so
	\begin{align*}
	\mathcal{A}_\epsilon^{ex}(\mu)[\varphi] &= \mathcal{A}_\epsilon(\mu)[\varphi] + \int_{-\epsilon}^{\epsilon}G_{\mathbb{R}^2\backslash\overline{\Omega}}^{\sqrt{\mu}}(x,y)\varphi(y)\mathrm{d}y \\
	&= -\frac{2}{\pi}\mathcal{L}_\epsilon[\varphi] + \frac{\mathcal{K}_\epsilon[\varphi]}{\mu_0-\mu} + (\mathcal{R}_\epsilon^0(\mu)[\varphi] + \int_{-\epsilon}^\epsilon r(x,y,\mu)\varphi(y)\mathrm{d}y).
	\end{align*}
	The final result follows if we define $\mathcal{R}_\epsilon(\mu)[\varphi]:=\mathcal{R}_\epsilon^0(\mu)[\varphi] + \int_{-\epsilon}^\epsilon r(x,y,\mu)\varphi(y)\mathrm{d}y$.
\end{proof}

With help of theorem \ref{thm:polepencildirichlet} and generalization of Steinberg theorem(Theorem 1.16 in \cite{LPTSA}), we could prove the following two important properties of characteristic value of $\mathcal{A}_\epsilon^{ex}$:

\begin{lemma}\label{lem:discretedirichlet}
	The set of characteristic values of $\mu\mapsto\mathcal{A}_\epsilon^{ex}(\mu)$ is discrete.
\end{lemma}
\begin{proof}
	Let $V$ be the same neighborhood of $\mu_0$ chosen in Lemma \ref{lem:dirichletexpansion}. We first prove the conclusion in $V$. Notice that $\mathcal{L}_\epsilon:\mathcal{X}^\epsilon\rightarrow\mathcal{Y}^\epsilon$ is invertible and $\|\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon\|_{\mathcal{L}(\mathcal{X}^\epsilon,\mathcal{X}^\epsilon)}\rightarrow 0$ as $\epsilon\rightarrow 0$. Therefore $-(2/\pi)\mathcal{L}_\epsilon + \mathcal{R}_\epsilon:\mathcal{X}^\epsilon\rightarrow\mathcal{Y}^\epsilon$ is invertible given $\epsilon$ small enough. We can then conclude from the decomposition \eqref{eq:polepencildirichlet} that $\mathcal{A}_\epsilon^{ex}$ is finitely meromorphic and of Fredholm type. In fact, $\frac{\mathcal{K}_\epsilon}{\mu_0-\mu}$ implies the pole of $\mathcal{A}_\epsilon^{ex}$ is order 1. Moreover, $\mathcal{A}_\epsilon^{ex}-\frac{\mathcal{K}_\epsilon}{\mu_0-\mu}$ is Fredholm because $\mathcal{L}_\epsilon:\mathcal{X}^\epsilon\rightarrow\mathcal{Y}^\epsilon_0$ is invertible and $\mathcal{R}_\epsilon$ is compact. Since $\mathcal{K}_\epsilon$ is finite dimension, there exists $\mu^*\in V$ such that $\mathcal{A}_\epsilon(\mu^*)$ is invertible. Therefore, the generalization of the Steinberg theorem gives the discreteness of set of characteristic values of $\mathcal{A}_\epsilon^{ex}$ in $V$. With the same method we could prove the result in each neighborhood $V_j$ of $\mu_j$, where $\mu_j$ is any eigenvalue to interior Dirichlet problem \eqref{eq:dirichlet}, and in $\mathbb{R}^2\backslash\bigcup_j V_j$.
\end{proof}

\begin{lemma}\label{lem:onechardirichlet}
	The operator-valued function $\mathcal{A}_\epsilon(\mu)$ has exactly one characteristic value in $V$, where $V$ is the same as Lemma \ref{lem:dirichletexpansion}.
\end{lemma}
\begin{proof}
	First we define the principal part of $\mathcal{A}_\epsilon^{ex}$:
	$$
		\mathcal{N}_\epsilon:=-\frac{2}{\pi}\mathcal{L}_\epsilon + \frac{\mathcal{K}_\epsilon}{\mu_0-\mu}.
	$$
	Now we would like to find the characteristic value of $\mathcal{N}_\epsilon$ in $V$. Suppose we have complex number $\tilde{\mu}$ and function $\tilde{\varphi}$ satisfying $\mathcal{N}_\epsilon(\tilde{\mu})[\tilde{\varphi}]=0$ on $(-\epsilon,\epsilon)$. $\tilde{\mu}$ and $\tilde{\varphi}$ then satisfies
	$$
		\frac{2}{\pi}\mathcal{L}_\epsilon[\tilde{\varphi}] + \frac{(\tilde{\varphi},u_{j0})}{\tilde{\mu}-\mu_0}u_{j0} = 0,
	$$
	which is
	$$
		\frac{2}{\pi}\tilde{\varphi} + \frac{(\tilde{\varphi},u_{j0})}{\tilde{\mu}-\mu_0}\mathcal{L}_\epsilon^{-1}[u_{j0}] = 0.
	$$
	Taking $L^2$ inner product on $(-\epsilon,\epsilon)$ on both side with $u_{j0}$, we have
	$$
		(\tilde{\varphi},u_{j0})\left(\frac{2}{\pi} + \frac{(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})}{\tilde{\mu}-\mu_0}\right) = 0,
	$$
	which means
	$$
		\tilde{\mu} = \mu_0 - \frac{\pi}{2}(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0}).
	$$
	Since $|(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})|\rightarrow 0$ as $\epsilon\rightarrow 0$, by choosing a sufficiently small $\epsilon$ we can always ensure that $\tilde{\mu}$ lies in $V$. The corresponding root function is 
	$$
		\tilde{\varphi} = \frac{\mathcal{L}_\epsilon^{-1}[u_{j0}]}{(\mathcal{L}_\epsilon^{-1}[u_{j0}], u_{j0})},
	$$
	if without loss of generality we assume $(\tilde{\varphi}, u_{j0}) =1$.
	Now we want to study the multiplicity of $\tilde{\mu}$ as a characteristic value of $\mathcal{N}_\epsilon$ in $V$. Suppose $\varphi$ and $f$ satisfies $\mathcal{N}_\epsilon(\mu)[\varphi]=f$, then
	$$
		-\frac{2}{\pi}\varphi + \frac{(\varphi,u_{j0})\mathcal{L}_\epsilon^{-1}[u_{j0}]}{\mu_0-\mu} = \mathcal{L}_\epsilon^{-1}[f].
	$$
	Therefore
	$$
		(\varphi,u_{j0})\left[-\frac{2}{\pi} + \frac{(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})}{\mu_0-\mu}\right] = (\mathcal{L}_\epsilon^{-1}[f],u_{j0}),
	$$
	which implies 
	$$
		(\varphi,u_{j0}) = \frac{\pi(\mu_0-\mu)}{2(\mu-\tilde{\mu})}(\mathcal{L}_\epsilon^{-1}[f],u_{j0}).
	$$
	We then have
	$$
	\varphi = -\frac{\pi}{2}\mathcal{L}_\epsilon^{-1}[f] + \frac{\pi^2}{4}\frac{(\mathcal{L}_\epsilon^{-1}[f],u_{j0})}{\mu-\tilde{\mu}}\mathcal{L}^{-1}_\epsilon[u_{j0}].
	$$
	Hence we could conclude that $\tilde{\mu}$ is the only characteristic value of $\mathcal{N}_\epsilon$ in $V$ and it is of order one.
	
	Now we examine the multiplicity of $\mathcal{A}_\epsilon^{ex}$ in $V$. It is obvious that $\mathcal{N}_\epsilon$ is normal and 
	$$
		\lim\limits_{\epsilon\rightarrow 0}\|\mathcal{N}_\epsilon^{-1}(\mu)\mathcal{R}_\epsilon(\mu)\|_{\mathcal{L}(\mathcal{X}^\epsilon,\mathcal{X}^\epsilon)} = 0, \quad\forall\mu\in\partial V.
	$$
	By generalized Rouch\'e theorem, $\mathcal{A}_\epsilon^{ex}$ has exactly one characteristic value $\mu^\epsilon$ in $V$.
\end{proof}

In view of Lemma \ref{lem:discretedirichlet}, Lemma \ref{lem:onechardirichlet} and Theorem \ref{thm:polepencildirichlet}, we could finally prove the main result of this chapter.
\begin{theorem}
	The operator-valued function $\mathcal{A}^{ex}_\epsilon(\mu)$ has exactly one characteristic value $\mu^\epsilon$ in $V$. Moreover, the following approximation of $\mu^\epsilon$ and $\varphi_\epsilon$ holds:
	\begin{equation}\label{eq:eigasymdirichlet}
	\mu^\epsilon=\mu_0-\pi(\mathcal{L}_\epsilon^{-1}[u_{j_0}],u_{j_0}) + \pi^2(\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon(\mu_0)\mathcal{L}_\epsilon^{-1}[u_{j_0}],u_{j_0}) + O(|\ln\epsilon|^{-2}) + O(|\ln\epsilon|^{-2}),
	\end{equation}
	\begin{equation}\label{eq:solasymdirichlet}
	\varphi_\epsilon = \frac{\mathcal{L}_\epsilon^{-1}[u_{j0}]}{(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})} + O(|\ln\epsilon|^{-1}).
	\end{equation}
\end{theorem}
\begin{proof}
	
	Denote $\varphi_\epsilon$ as the corresponding root function of $\mathcal{A}^{ex}_\epsilon(\mu)$. Therefore we have
	\begin{equation}
	\frac{1}{\pi}\mathcal{L}_\epsilon[\varphi_\epsilon] + \frac{(\varphi_\epsilon,u_{j0})}{\mu_\epsilon-\mu_0}u_{j0} - \mathcal{R}_\epsilon[\varphi_\epsilon]=0.
	\end{equation}
	By Lemma 5.2 in \cite{LPTSA}, $\mathcal{L}_\epsilon$ is invertible. Therefore
	\begin{equation}\label{eq:varphi1d}
	\frac{1}{\pi}\varphi_\epsilon + \frac{(\varphi_\epsilon,u_{j0})}{\mu_\epsilon-\mu_0}\mathcal{L}_\epsilon^{-1}[u_{j0}] - \mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon[\varphi_\epsilon]=0.
	\end{equation}
	Taking inner product against $u_{j0}$ on both side, we get
	\begin{equation}
	\frac{1}{\pi} + \frac{(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})}{\mu_\epsilon-\mu_0} - (\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon[\varphi_\epsilon],u_{j0}) = 0,
	\end{equation}
	that is,
	\begin{equation}\label{eq:equation4d}
	\mu_\epsilon - \mu_0 + \pi(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})-\pi(\mu_\epsilon-\mu_0)(\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon[\varphi_\epsilon],u_{j0}) =0.
	\end{equation}
	Since $\|\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon\|_{\mathcal{L}(\mathcal{X}^\epsilon,\mathcal{X}^\epsilon)}\leq\frac{C}{\ln\epsilon}$, and $\mathcal{L}_\epsilon^{-1}[u_{j0}] = O(|\ln\epsilon|^{-1})$, we know $\mu_\epsilon - \mu_0 = O(|\ln\epsilon|^{-1})$. Plug it back into \eqref{eq:equation4d}, we have that
	\begin{equation}\label{eq:equation5d}
	\mu_\epsilon - \mu_0 = -\pi(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0}) + O(|\ln\epsilon|^{-2}).
	\end{equation}
	Meanwhile, from \eqref{eq:varphi1d} it follows that
	\begin{equation}\label{eq:varphi2d}
	\varphi_\epsilon = -\frac{\pi}{\mu_\epsilon-\mu_0}\mathcal{L}_\epsilon^{-1}[u_{j0}]+\pi \mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon[\varphi_\epsilon]
	\end{equation}
	Combining \eqref{eq:equation4d} and \eqref{eq:varphi2d} implies
	\begin{equation}\label{eq:dirichleteigexpansion}
	\mu_\epsilon = \mu_0 -\pi(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0}) + \pi^2(\mathcal{L}_\epsilon^{-1}\mathcal{R}_\epsilon\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0}) + O(|\ln\epsilon|^{-2}).
	\end{equation}
	Combining \eqref{eq:equation5d} and \eqref{eq:varphi1d} leads to
	\begin{equation}\label{eq:dirichletsolexpansion}
	\varphi_\epsilon = \frac{\mathcal{L}_\epsilon^{-1}[u_{j0}]}{(\mathcal{L}_\epsilon^{-1}[u_{j0}],u_{j0})} + O(|\ln\epsilon|^{-1}).
	\end{equation}
\end{proof}

\section{Error Estimation and Numerical Implementation}

In this section we will numerically implement the result in previous chapter. Given a domain $\Omega$, a source at $x_S\in\Omega$ and a receiver at $x_R\in\Omega$, we will rotate the small opening $\partial\Omega_N$ on $\partial\Omega$ and regard $u_{x_S}^{k,\epsilon}$ in Theorem \ref{thm:ch4mainresult} as a function of $\theta$, i.e. the position angle of $\partial\Omega_N$. Empirically we believe that if we switch the place with positive $\frac{\partial}{\partial\theta}u_{x_S}^{k,\epsilon}$ from Dirichlet boundary to Neumann boundary,  $u_{x_S}^{k,\epsilon}(x_R)$ will be magnified compared to a pure Dirichlet case. We will plot $\frac{\partial}{\partial\theta}u_{x_S}^{k,\epsilon}$ and give boundary configuration with different $x_S$, $x_R$ locations.


Here we will make some simplifications to the settings in previous chapter. $\Omega$ will be a unit 2-dimensional disk with radius 1 centered at origin. The coordinate of source and receiver is $x_S=(x,y)$ and $x_R=(\xi,\eta)$. The opening $\partial\Omega_N$ is an arc centered at $(1,0)$ with length $2\epsilon$. In simulation we approximate the arc by a short segment between $(-\epsilon,1)$ and $(\epsilon,1)$. 

Denote $\rho=\sqrt{x^2+y^2}$ as the distance between $x_S$ and origin, and $\tilde{\rho}=\sqrt{\xi^2+\eta^2}$ as the distance between $x_R$ and origin. Define $\theta = \arctan(y/x)$, and $\tilde{\theta} = \arctan(\eta/\xi)$. It is well-known that Green's function satisfies 2-dimensional Helmholtz equation in unit disk could be written in the form of
\begin{equation}\label{eq:num1}
G_\Omega^k(x_S,x_R) = -\frac{i}{4}H_0^{(1)}(k|x_S-x_R|) + \frac{i}{4}\sum\limits_{n=-\infty}^{+\infty}A_n(k,\rho)J_n(k\tilde\rho)e^{in(\theta-\tilde{\theta})}.
\end{equation}
The cylinder wave expansion for free-boundary Green's function is 
\begin{equation}\label{eq:num2}
-\frac{i}{4}H_0^{(1)}(k|x_S-x_R|) = -\frac{i}{4}\sum\limits_{n=-\infty}^{+\infty}J_n(k\rho_<)H_n^{(1)}(k\rho_>)e^{in(\theta-\tilde{\theta})}
\end{equation}
where $\rho_< = \min(\rho,\tilde{\rho})$, $\rho_>=\max(\rho,\tilde{\rho})$. Substitute \eqref{eq:num2} into \eqref{eq:num1} gives
\begin{equation}\label{eq:num3}
G_\Omega^k(x_S,x_R) = \frac{i}{4}\sum\limits_{n=-\infty}^\infty(A_nJ_n(k\rho)-J_n(k\rho_<)H_n^{(1)}(k\rho_>))e^{in(\theta-\tilde{\theta})}.
\end{equation}
Imposing Dirichlet boundary condition on \eqref{eq:num3} yields
$$
A_n(k,\rho) = \frac{J_n(k\rho)H_n^{(1)}(k)}{J_n(k)},
$$
and Green's function is
\begin{equation}\label{eq:greendisk}
G_\Omega^k(x_S,x_R) = -\frac{i}{4}H_0^{(1)}(k|x_S-x_R|)+\frac{i}{4}\sum\limits_{n=-\infty}^\infty\frac{J_n(k\rho)H_n^{(1)}(k)}{J_n(k)}J_n(k\tilde{\rho}),
\end{equation}
and its normal derivative on $\partial\Omega_N$ is
\begin{equation}\label{eq:greenderivative}
\begin{aligned}
\frac{\partial G_\Omega^k}{\partial\tilde\rho}\left(x_S,\begin{pmatrix}t \\ 1 \end{pmatrix}\right) =& -\frac{i}{4}kH_0^{(1)'}(k\sqrt{\rho^2+1-2\rho\cos(\theta-\theta_0)})\frac{1-\rho\cos(\theta-\theta_0)}{\sqrt{\rho^2+1-2\rho\cos(\theta-\theta_0)}} \\
& + \frac{i}{4}\sum\limits_{n=-\infty}^\infty\frac{J_n(k\rho)H_n^{(1)}(k)}{J_n(k)}kJ_n'(k) ,
\end{aligned}
\end{equation}
where $\arctan\theta_0 = 1/t$. By properties of Hankel function, we could use the following recurrence property to calculate derivative to $H_0^{(1)}$:
$$
2\frac{\mathrm{d}H_\alpha^{(1)}}{\mathrm{d}x} = \frac{1}{2}(H_{\alpha-1}^{(1)}(x) - H_{\alpha+1}^{(1)}(x)).
$$

We would like to examine the value of $u_{x_S}^{k,\epsilon}$ given fixed source, receiver position and different opening position. In simulation, we will fix the opening to be the segment between $(-\epsilon,1)$ and $(\epsilon,1)$, but rotate $x_S$ and $x_R$. That is, $\theta$ and $\tilde{\theta}$ will vary while $\rho$, $\tilde{\rho}$, $\theta-\tilde{\theta}$ remain unchanged. From now on we will focus on the estimation to $\frac{\partial u_{x_S}^{k,\epsilon}}{\partial\theta}$.

From \eqref{eq:uxs}, $u_{x_S}^{k,\epsilon}$ consists of two parts. The first part $G_\Omega^k(x_S,x_R)$ does not change because $\rho$, $\tilde{\rho}$ and $\theta-\tilde{\theta}$ remain unchanged, therefore we only need to care about the second part. Define

$$
I_1:=\int_{-\epsilon}^{\epsilon}\partial_{\nu_y}G_\Omega^k\left(x_R,\begin{pmatrix}
t \\ 1
\end{pmatrix}\right)(-\frac{1}{2\pi}\mathcal{J}^\epsilon + \frac{k^2}{4\pi}\mathcal{L}^\epsilon)^{-1}\left[\partial_{\nu_x}G_\Omega^k\left(x_S,\begin{pmatrix}
s \\ 1
\end{pmatrix}\right)\right](t)\mathrm{d}t.
$$
We will try to find out the main part of $I_1$ in the following section.

\subsubsection{Estimation of $I_1$}

By Proposition \ref{prop:-aLLe+bJJeInverse}, we have
$$
(-\alpha\mathcal{J}^\epsilon + \beta\mathcal{L}^\epsilon)^{-1}[f](t) = (\mathcal{L}^\epsilon)^{-1}[u_l](t),
$$
where
$$
u_l(t) = C_1e^{\sqrt{\frac{\beta}{\alpha}}t} + C_2e^{-\sqrt{\frac{\beta}{\alpha}}t} + \frac{1}{2\sqrt{\alpha\beta}}e^{-\sqrt\frac{\beta}{\alpha}t}\int_{-\epsilon}^tf(s)e^{\sqrt\frac{\beta}{\alpha}s}\mathrm{d}s - \frac{1}{2\sqrt{\alpha\beta}}e^{\sqrt\frac{\beta}{\alpha}t}\int_{-\epsilon}^tf(s)e^{-\sqrt\frac{\beta}{\alpha}s}\mathrm{d}s,
$$
and $C_1$, $C_2$ are constants determined by \eqref{equ:-aLLe+bJJeInverse:SOE:1} and \eqref{equ:-aLLe+bJJeInverse:SOE:2}.	With direct calculation, we learn that
$$
u_l'(\tau) = \sqrt\frac{\beta}{\alpha}\left(C_1e^{\sqrt{\frac{\beta}{\alpha}}\tau} - C_2e^{-\sqrt{\frac{\beta}{\alpha}}\tau}-\frac{1}{2\sqrt{\alpha\beta}}\int_{-\epsilon}^\tau f(s)2\cosh(\sqrt\frac{\beta}{\alpha}(s-\tau))\mathrm{d}s\right).
$$
By using Taylor expansion, we calculate the error from substituting $u_l'(\tau)$ with $u_l'(0)$ as follows
\begin{equation}\label{eq:ulderivative}
\begin{aligned}
&u_l'(\tau) - u_l'(0) \\
=& \sqrt{\frac{\beta}{\alpha}}(C_1e^{\sqrt{\frac{\beta}{\alpha}}\tau} - C_2e^{-\sqrt{\frac{\beta}{\alpha}}\tau} - (C_1-C_2)) - \frac{1}{2\alpha}\int_0^\tau f(s)2\cosh(\sqrt\frac{\beta}{\alpha}(s-\tau))\mathrm{d}s \\
&-\frac{1}{2\alpha}\int_{-\epsilon}^0f(s)2\left(\cosh(\sqrt{\frac{\beta}{\alpha}}(s-\tau))-\cosh(\sqrt{\frac{\beta}{\alpha}}s)\right)\mathrm{d}s \\
=& \sqrt{\frac{\beta}{\alpha}}\left(C_1\sqrt{\frac{\beta}{\alpha}} + C_2\sqrt{\frac{\beta}{\alpha}}\right)\tau + \frac{1}{2}\left(\frac{\beta}{\alpha}\right)^{3/2}(C_1-C_2)\tau^2 \\
&- \frac{1}{2\alpha}\left(2f(0)\tau + f'(0)\tau^2 + \frac{\beta}{\alpha}f(0)\tau^2\epsilon + \frac{\beta}{\alpha}f(0)\tau\epsilon^2 + O(\tau^3)\right) \\
=& \left(\frac{\beta}{\alpha}(C_1+C_2)\tau - \frac{1}{\alpha}f(0)-\frac{\beta}{2\alpha^2}f(0)\epsilon^2\right)\tau \\
&+ \left(\frac{1}{2}\left({\frac{\beta}{\alpha}}\right)^{3/2}(C_1-C_2) - \frac{1}{2\alpha}f'(0) - \frac{\beta}{2\alpha^2}f(0)\epsilon\right)\tau^2 + O(\tau^3).
\end{aligned}
\end{equation}
Denote 
\begin{equation}\label{eq:cul1}
C_{u_l}^1 := \frac{\beta}{\alpha}(C_1+C_2) - \frac{1}{\alpha}f(0) - \frac{\beta}{2\alpha^2}f(0)\epsilon^2
\end{equation}
and
\begin{equation}\label{eq:cul2}
C_{u_l}^2 := \frac{1}{2}\left({\frac{\beta}{\alpha}}\right)^{3/2}(C_1-C_2) - \frac{1}{2\alpha}f'(0) - \frac{\beta}{2\alpha^2}f(0)\epsilon.
\end{equation}
On the other hand, for $u_l'(0)$ we have
\begin{equation}\label{eq:ul0derivative}
\begin{aligned}
u_l'(0) =& \sqrt{\frac{\beta}{\alpha}}\left(C_1-C_2-\frac{1}{2\sqrt{\alpha\beta}}\int_{-\epsilon}^0 f(s)2\cosh(\sqrt{\frac{\beta}{\alpha}}s)\mathrm{d}s\right) \\
=& \sqrt{\frac{\beta}{\alpha}}(C_1-C_2 \\
&- \frac{1}{\sqrt{\alpha\beta}}\left(f(0)\sqrt{\frac{\alpha}{\beta}}\sinh(\sqrt\frac{\beta}{\alpha}\epsilon) + f'(0)\frac{\alpha}{\beta}\left(-1+\cosh(\sqrt{\frac{\beta}{\alpha}}\epsilon)-\epsilon\sqrt{\frac{\beta}{\alpha}}\sinh(\sqrt{\frac{\beta}{\alpha}}\epsilon)\right)+ O(\epsilon^3)\right) \\
=& \sqrt\frac{\beta}{\alpha}(C_1-C_2) - \frac{1}{\alpha}f(0)\epsilon + \frac{1}{2\alpha}f'(0)\epsilon^2+ O(\epsilon^3),
\end{aligned}
\end{equation}
and for $u_l(0)$ it holds that
\begin{equation}\label{eq:ul0}
\begin{aligned}
u_l(0) &= C_1 + C_2 + \frac{1}{2\sqrt{\alpha\beta}}\int_{-\epsilon}^0 f(s)(e^{\sqrt\frac{\beta}{\alpha}s} - e^{-\sqrt\frac{\beta}{\alpha}s})\mathrm{d}s \\
&= C_1 + C_2 + \frac{1}{\alpha}f(0)(-\frac{1}{2}\epsilon^2) + O(\epsilon^4)
\end{aligned}
\end{equation}
Recall the formula for $(\mathcal{L}^\epsilon)^{-1}$ and $C_{\mathcal{L}^\epsilon}[u_l]$ in Proposition \ref{prop:LLEisInjective}. Since $C_{\mathcal{L}^\epsilon}[u_l]$ is a constant, we could actually take value at any point on the right hand side of \eqref{eq:cl}. Here we take $x=0$, and
\begin{align*}
C_{\mathcal{L}^\epsilon}[u_l] &= u_l(0) - \mathcal{L}^\epsilon[-\frac{1}{\pi^2\sqrt{\epsilon^2-t^2}}\int_{-\epsilon}^{\epsilon}\frac{\sqrt{\epsilon^2-\tau^2}u_l'(\tau)}{t-\tau}\mathrm{d}\tau](0) \\
&= u_l(0) - \int_{-\epsilon}^\epsilon\int_{-\epsilon}^\epsilon - \frac{1}{\pi^2\sqrt{\epsilon^2-t^2}}\frac{\sqrt{\epsilon^2-\tau^2}u_l'(\tau)}{t-\tau}\log|t|\mathrm{d}\tau\mathrm{d}t	
\end{align*}
Applying the result from \eqref{eq:ulderivative}, we have 
\begin{align*}
&\int_{-\epsilon}^\epsilon\int_{-\epsilon}^\epsilon - \frac{1}{\pi^2\sqrt{\epsilon^2-t^2}}\frac{\sqrt{\epsilon^2-\tau^2}u_l'(\tau)}{t-\tau}\log|t|\mathrm{d}\tau\mathrm{d}t \\
=&\int_{-\epsilon}^\epsilon\int_{-\epsilon}^\epsilon- \frac{1}{\pi^2\sqrt{\epsilon^2-t^2}}\frac{\sqrt{\epsilon^2-\tau^2}(u_l'(0) + C_{u_l}^1\tau + C_{u_l}^2\tau^2 + O(\epsilon^3)) }{t-\tau}\log|t|\mathrm{d}\tau\mathrm{d}t  \\
=&-u_l'(0)\int_{-\epsilon}^\epsilon \frac{1}{\pi^2\sqrt{\epsilon^2-t^2}}\pi t\log|t|\mathrm{d}t - C_{u_l}^1\int_{-\epsilon}^\epsilon\frac{1}{\pi^2\sqrt{\epsilon^2-t^2}}(-\frac{\pi\epsilon^2}{2} + \pi t^2)\log|t|\mathrm{d}t \\
& - C_{u_l}^2\int_{-\epsilon}^\epsilon\frac{}{\pi^2\sqrt{\epsilon^2-t^2}}(-\frac{1}{2}\epsilon^2\pi t + \pi t^3)\log|t|\mathrm{d}t + O(\epsilon^4) \\
=& 0 - \frac{C_{u_l}^1}{\pi}\left(-\frac{\epsilon^2}{2}(-\pi\log(\frac{2}{\epsilon}))-\frac{1}{4}\epsilon^2\pi(-1+2\log(\frac{2}{\epsilon}))\right) + 0 + O(\epsilon^4) \\
=& -\frac{C_{u_l}^1}{4}\epsilon^2 + O(\epsilon^4),
\end{align*}
where we have used the fact that 
$$
p.v.\int_{-\epsilon}^\epsilon\frac{\tau\sqrt{\epsilon^2-\tau^2}}{t-\tau}\mathrm{d}\tau = -\frac{\pi\epsilon^2}{2} + \pi t^2,
$$
$$
\int_{-\epsilon}^\epsilon\frac{\log|t|}{\sqrt{\epsilon^2-t^2}}\mathrm{d}t = -\pi\log\left(\frac{2}{\epsilon}\right),
$$
and
$$
\int_{-\epsilon}^\epsilon \frac{t^2\log|t|}{\sqrt{\epsilon^2-t^2}}\mathrm{d}t = -\frac{1}{4}\epsilon^2\pi\left(-1+2\log\left(\frac{2}{\epsilon}\right)\right).
$$
Therefore the following estimation holds
\begin{equation}\label{eq:clepsilonest}
C_{\mathcal{L}^\epsilon}[u_l] = u_l(0) + \frac{C_{u_l}^1}{4}\epsilon^2 + O(\epsilon^4).
\end{equation}
The last preparation is to solve $C_1$ and $C_2$ out of equation \eqref{equ:-aLLe+bJJeInverse:SOE:1} and \eqref{equ:-aLLe+bJJeInverse:SOE:2}. Apply \eqref{eq:ulderivative} to \eqref{equ:-aLLe+bJJeInverse:SOE:1} we get
$$
\int_{-\epsilon}^\epsilon\sqrt\frac{\epsilon+\tau}{\epsilon-\tau}(u_l'(0) + C_{u_l}^1\tau + C_{u_l}^2\tau^2 + O(\tau^3))\mathrm{d}\tau - \frac{\pi}{\log(\epsilon/2)}C_{\mathcal{L}^\epsilon}[u_l] = 0,
$$
which implies
$$
u_l'(0)\pi\epsilon + C_{u_l}^1\frac{\pi\epsilon^2}{2} + C_{u_l}^2\frac{\pi\epsilon^3}{2}  - \frac{\pi}{\log(\epsilon/2)}(u_l(0) + \frac{C_{u_l}}{4}\epsilon^2) +O(\epsilon^4)= 0.
$$
Combine last equation with \eqref{eq:ul0} and \eqref{eq:ul0derivative}, it follows that
\begin{equation}
\begin{aligned}
&\left(\sqrt\frac{\beta}{\alpha}(C_1-C_2) - \frac{1}{\alpha}f(0)\epsilon + O(\epsilon^2)\right)\pi\epsilon + C_{u_l}^1\frac{\pi\epsilon^2}{2} + C_{u_l}^2\frac{\pi\epsilon^3}{2} + O(\epsilon^4) \\
&- \frac{\pi}{\log(\epsilon/2)}\left(C_1 + C_2 - \frac{1}{2\alpha}f(0)\epsilon^2 + O(\epsilon^4) + \frac{C_{u_l}}{4}\epsilon^2\right) = 0.
\end{aligned}
\end{equation}
Reorganizing terms gives 
\begin{equation}
\begin{aligned}
\sqrt\frac{\beta}{\alpha}\epsilon(C_1 - C_2) &- \frac{1}{\log(\epsilon/2)}(C_1 + C_2) \\
&= 
\frac{1}{\alpha}f(0)\epsilon^2 -\frac{C_{u_l}^1}{2}\epsilon^2 - \frac{C_{u_l}^2}{2}\epsilon^3- \frac{1}{\log(\epsilon/2)}\left(\frac{1}{2\alpha}f(0)\epsilon^2 - \frac{C_{u_l}}{4}\epsilon^2\right) + O(\epsilon^4).
\end{aligned}
\end{equation}
With same reasoning, from Equation \eqref{equ:-aLLe+bJJeInverse:SOE:2} we have
\begin{equation}
\begin{aligned}
-\sqrt\frac{\beta}{\alpha}\epsilon(C_1 - C_2) &- \frac{1}{\log(\epsilon/2)}(C_1 + C_2) \\
&= 
-\frac{1}{\alpha}f(0)\epsilon^2 - \frac{C_{u_l}^1}{2}\epsilon^2 + \frac{C_{u_l}^2}{2}\epsilon^3- \frac{1}{\log(\epsilon/2)}\left(\frac{1}{2\alpha}f(0)\epsilon^2 - \frac{C_{u_l}}{4}\epsilon^2\right) + O(\epsilon^4).
\end{aligned}
\end{equation}
Therefore,
\begin{equation}\label{eq:c1plusc2}
C_1 + C_2 =\left(\frac{1}{2\alpha}f(0)-  \frac{C_{u_l}^1}{4}\right)\epsilon^2 + \frac{C_{u_l}^1}{2}\log(\epsilon/2)\epsilon^2 + O(\epsilon^3),
\end{equation}
and
\begin{equation}\label{eq:c1minusc2}
C_1 - C_2 = \frac{1}{\sqrt{\alpha\beta}}f(0)\epsilon - \frac{1}{2}\sqrt{\frac{\alpha}{\beta}}C_{u_l}^2\epsilon^2+ O(\epsilon^2).
\end{equation}

\eqref{eq:cul1} and \eqref{eq:c1plusc2} together gives
\begin{equation}\label{eq:c1plusc2final}
\begin{aligned}
C_1 + C_2 &= \frac{\frac{-1}{2\alpha}f(0)\log(\epsilon/2)\epsilon^2 + \frac{3}{4\alpha}f(0)\epsilon^2}{1-\frac{\beta}{2\alpha}\log(\epsilon/2)\epsilon^2+\frac{\beta}{4\alpha}\epsilon^2} + O(\epsilon^3\log\epsilon) \\
&= -\frac{1}{2\alpha}f(0)\log(\epsilon/2)\epsilon^2 + \frac{3}{4\alpha}f(0)\epsilon^2 + O(\epsilon^2\log\epsilon)
\end{aligned}
\end{equation}
and
\begin{equation}\label{eq:cul1final}
C_{u_l}^1 = -\frac{1}{\alpha}f(0) + \frac{\beta}{\alpha}\left(-\frac{1}{2\alpha}f(0)\log(\epsilon/2)\epsilon^2 + \frac{3}{4\alpha}f(0)\epsilon^2\right) + O(\epsilon^2\log\epsilon),
\end{equation}
while \eqref{eq:cul2} and \eqref{eq:c1minusc2} together gives
\begin{equation}\label{eq:c1minusc2final}
C_1 - C_2 = \frac{1}{\sqrt{\alpha\beta}}f(0)\epsilon + \frac{1}{4\sqrt{\alpha\beta}}f'(0)\epsilon^2 + O(\epsilon^3)
\end{equation}
and
\begin{equation}\label{eq:cu2final}
C_{u_l}^2 = -\frac{1}{2\alpha}f'(0) + \frac{1}{8\alpha^2}f'(0)\epsilon^2 + O(\epsilon^3).
\end{equation}
Now we are ready to estimate $(\mathcal{L}_\epsilon)^{-1}[u_l](t)$. From Proposition \ref{prop:LLEisInjective}, we know that
\begin{equation}
\begin{aligned}
(\mathcal{L}_\epsilon)^{-1}[u_l](t) &= -\frac{1}{\pi^2\sqrt{\epsilon^2-t^2}}p.v.\int_{-\epsilon}^\epsilon\frac{\sqrt{\epsilon^2-\tau^2}u_l'(\tau)}{t-\tau}\mathrm{d}\tau + \frac{C_{\mathcal{L}^\epsilon}[u_l]}{\pi\log(\epsilon/2)\sqrt{\epsilon^2-t^2}} \\
&= -\frac{1}{\pi^2\sqrt{\epsilon^2-t^2}}\int_{-\epsilon}^\epsilon\frac{\sqrt{\epsilon^2-\tau^2}(u_l'(0)+C_{u_l}^1\tau + C_{u_l}^2\tau^2+ O(\tau^3))}{t-\tau}\mathrm{d}\tau + \frac{C_{\mathcal{L}^\epsilon}[u_l]}{\pi\log(\epsilon/2)\sqrt{\epsilon^2-t^2}} \\
&= -\frac{1}{\pi\sqrt{\epsilon^2-t^2}}u_l'(0)t - \frac{C_{u_l}^1}{\pi\sqrt{\epsilon^2-t^2}}(-\frac{1}{2}\epsilon^2 + \frac{1}{2}t^2) -\frac{C_{u_l}^2}{\pi\sqrt{\epsilon^2-t^2}}(-\frac{1}{2}\epsilon^2\pi t + \pi t^3)+ O(\epsilon^4).
\end{aligned}
\end{equation}
Plug \eqref{eq:ul0derivative}, $\alpha = 1/(2\pi)$ and $\beta = k^2/(4\pi)$ into equation and get
\begin{equation}
\begin{aligned}
&\left(-\frac{1}{2\pi}\mathcal{J}^\epsilon + \frac{k^2}{4\pi}\mathcal{L}^\epsilon\right)^{-1}[f](t) \\
=& -\frac{1}{\sqrt{\epsilon^2-t^2}}\left( -f(0)t^2 - f'(0)\pi t^3 +f(0)\epsilon^2 + \frac{1}{2}f'(0)\epsilon^2\pi t + \frac{3}{2}f'(0)\epsilon^2 t + O(\epsilon^3)\right).
\end{aligned}
\end{equation}
Therefore
\begin{equation}
\begin{aligned}
&\int_{-\epsilon}^{\epsilon}\partial_{\nu_y}G_\Omega^k(x_R,\begin{pmatrix}
t \\ 1
\end{pmatrix})(-\frac{1}{2\pi}\mathcal{J}^\epsilon + \frac{k^2}{4\pi}\mathcal{L}^\epsilon)^{-1}[f](t)\mathrm{d}t \\
=&\left(2\epsilon\partial_{\nu_y}G_\Omega^k\left(x_R,\begin{pmatrix}
0 \\ 1
\end{pmatrix}\right)+O(\epsilon^2)\right)\\
&\int_{-\epsilon}^{\epsilon}-\frac{1}{\sqrt{\epsilon^2-t^2}}\left( -f(0)t^2 - f'(0)\pi t^3 +f(0)\epsilon^2 + \frac{1}{2}f'(0)\epsilon^2\pi t + \frac{3}{2}f'(0)\epsilon^2 t + O(\epsilon^3)\right)\mathrm{d}t \\
=&\left(2\epsilon\partial_{\nu_y}G_\Omega^k\left(x_R,\begin{pmatrix}
0 \\ 1
\end{pmatrix}\right)+O(\epsilon^2)\right)\left(f(0)\frac{\epsilon^2\pi}{2}-f(0)\epsilon^2\pi+O(\epsilon^3)\right) \\
=& -f(0)\pi\epsilon^3\partial_{\nu_y}G_\Omega^k\left(x_R,\begin{pmatrix}
0 \\ 1
\end{pmatrix}\right) + O(\epsilon^4)
\end{aligned}
\end{equation}
Recall in our setting, $f(s):=\partial_{\nu_x}G_\Omega^k\left(x_S,\begin{pmatrix}
s \\ 1
\end{pmatrix}\right)$, thus
\begin{equation}
\begin{aligned}
&\int_{-\epsilon}^{\epsilon}\partial_{\nu_y}G_\Omega^k\left(x_R,\begin{pmatrix}
t \\ 1
\end{pmatrix}\right)\left(-\frac{1}{2\pi}\mathcal{J}^\epsilon + \frac{k^2}{4\pi}\mathcal{L}^\epsilon\right)^{-1}\left[\partial_{\nu_x}G_\Omega^k\left(x_S,\begin{pmatrix}
s \\ 1
\end{pmatrix}\right)\right](t)\mathrm{d}t \\
&=-\pi\epsilon^3\partial_{\nu_x}G_\Omega^k\left(x_S,\begin{pmatrix}
0 \\ 1
\end{pmatrix}\right)\partial_{\nu_y}G_\Omega^k\left(x_R,\begin{pmatrix}
0 \\ 1
\end{pmatrix}\right) + O(\epsilon^4)
\end{aligned}
\end{equation}

\subsubsection{Numerical Implementation}

Denote 
\begin{equation}\label{eq:deffs}
F_S(\theta):=\frac{\partial G_\Omega^k}{\partial\tilde\rho}\left(x_S,\begin{pmatrix}0 \\ 1\end{pmatrix}\right),
\end{equation}
and 
\begin{equation}
\label{eq:deffr}
F_R(\theta):=\frac{\partial G_\Omega^k}{\partial\tilde\rho}\left(x_R,\begin{pmatrix}0 \\ 1 \end{pmatrix}\right).
\end{equation}

\iffalse
Define $d_S(\theta):= \sqrt{\rho^2+1-2\rho\cos(\theta-\pi/2)}$, and $d_R(\theta):=\sqrt{\tilde{\rho}^2+1-2\tilde\rho\cos(\tilde{\theta}-\pi/2)}$. Then
\begin{equation}\label{eq:dfs}
\begin{aligned}
\frac{\mathrm{d}}{\mathrm{d}\theta}F_S(\theta) =& -\frac{i}{4}k\left(\frac{1}{2}(H_{-1}^{(1)}(kd_S(\theta))-H_1^{(1)}(kd_S(\theta)))\frac{\rho\sin(\theta-\pi/2)d_S(\theta)-d_S'(\theta)(1-\rho\cos(\theta-\pi/2))}{d_S^2(\theta)}\right. \\
&\left.+\frac{1}{4}(H_{-2}^{(1)}(kd_S(\theta))-2H_0^{(1)}(kd_S(\theta))+H_2^{(1)}(kd_S(\theta)))kd_S'(\theta)\frac{1-\rho\cos(\theta-\pi/2)}{d_S(\theta)}\right)
\end{aligned}
\end{equation}
By replacing $\rho$ with $\tilde{\rho}$ and $\theta$ with $\tilde{\theta}$ we have a similar formula for $\frac{\mathrm{d}}{\mathrm{d}\theta}F_R(\theta)$. As a conclusion, we have proved that

\begin{theorem}\label{thm:numerical}
	Let $\Omega$ is a 2-dimensional disk. When regarding $u_{x_S}^{k,\epsilon}(x_R)$ as a function of $\theta$, it holds that
	\begin{equation}
	\frac{\partial}{\partial\theta}u_{x_S}^{k,\epsilon}(x_R) = \pi\epsilon^3\left(\frac{\mathrm{d}F_S(\theta)}{\mathrm{d}\theta}F_R(\theta) + \frac{\mathrm{d}F_R(\theta)}{\mathrm{d}\theta}F_S(\theta)\right) + O(\epsilon^4),
	\end{equation}
	where $F_S(\theta)$ and $F_R(\theta)$ are defined in \eqref{eq:deffs} and \eqref{eq:deffr}.
\end{theorem}

\begin{remark}
	Notice Theorem \ref{thm:numerical} has a finer result than Theorem \ref{thm:ch4mainresult}. The main reason is that here we know the explicit formula of Green's function $G_\Omega^k(x,y)$, and in fact it is smooth whenever $x\neq y$. We did Taylor expansion for a higher order as estimation instead of using $C^{0,\alpha}$ norm, which results in a finer result.
	
	Another important remark is, although the order of 
	$$
		\int_{-\epsilon}^\epsilon\partial_{\nu_y}G_\Omega^k\left(x_R,\begin{pmatrix}t \\ 0\end{pmatrix}\right)\left(-\frac{1}{2\pi}\mathcal{J}^\epsilon + \frac{k^2}{4\pi}\mathcal{L}^\epsilon\right)^{-1}\left[\partial_{\nu_x}G_\Omega^k\left(x_S,\begin{pmatrix}\tau \\ 0\end{pmatrix}\right)\right](t)\mathrm{d}t
	$$
	is finer than Theorem \ref{thm:ch4mainresult}, the order of remainder here is also finer than the one in Theorem \ref{thm:ch4mainresult} so Equation \eqref{eq:uxs} is still applicable.
\end{remark}




In numerical implementation, we plot a graph with $\theta$ from $0$ to $2\pi$ as x-axis and $\frac{\partial}{\partial\theta}u_{x_S}^{k,\epsilon}$ as y-axis. Notice that although the term
$$
\sum\limits_{n=-\infty}^\infty\frac{J_n(k\rho)H_n^{(1)}(k)}{J_n(k)}kJ_n'(k)
$$
is an infinite sum, we could truncate the sum between $n=-100$ and $n=100$ since all summand outside this range are negligible. The following plot shows the norm of $\frac{J_n(k\rho)H_n^{(1)}(k)}{J_n(k)}kJ_n'(k)$ from $n=-1000$ to $n=1000$ with $\rho=0.4$ and $k=200$.
\begin{figure}[ht!]
	\centering
	\includegraphics[scale=0.5]{Images/norm.eps}
	\caption{Norm of $\frac{J_n(k\rho)H_n^{(1)}(k)}{J_n(k)}kJ_n'(k)$ from $n=-1000$ to $n=1000$}
	\label{fig:remaindernorm}
\end{figure}

Recall we denote $\theta$ as the angle from x-axis to source, and $\tilde{\theta}$ as the angle from x-axis to receiver. The next two plots(Figure \ref{fig:derivativeuxs1} and Figure \ref{fig:derivativeuxs2}) show us the relationship between $\theta$ and $\frac{\partial}{\partial\theta}u_{x_S}^{k,\epsilon}$ when we set: (i): $\rho=0.2$, $\tilde{\rho}=0.3$, $\tilde{\theta}-\theta = \pi/4$, opening length $2\epsilon=0.02$ and wave number $k=200$; (ii): $\rho = 0.4$, $\tilde{\rho}=0.2$, $\tilde{\theta}-\theta = \pi/3$, opening length $2\epsilon=0.02$ and wave number $k=200$.

\begin{figure}[ht!]
	\centering
	\includegraphics[scale=0.5,width=\textwidth]{Images/ri1.eps}
	\caption{Graph of $\frac{\partial}{\partial\theta}u_{x_S}^{k,\epsilon}$ in Setting (i)}
	\label{fig:derivativeuxs1}
\end{figure}

\begin{figure}[ht!]
	\centering
	\includegraphics[scale=0.5,width=\textwidth]{Images/ri2.eps}
	\caption{Graph of $\frac{\partial}{\partial\theta}u_{x_S}^{k,\epsilon}$ in Setting (ii)}
	\label{fig:derivativeuxs2}
\end{figure}
In practice, in order to make smart wall magnify the signal at receiver, we would like to keep all the positive derivative part as opening(Neumann boundary), and all negative derivative part as wall(Dirichlet boundary). One last thing we should care about is the assumption we made at the very beginning of this section. In our implementation we set opening to be fixed and receiver is rotating along with source, while in practical setting receiver and source are fixed. If we set the source to always stay on x-axis, then the actual angle of opening $\theta_0 = \pi/2-\theta$. With the same setting (i) and (ii) as mentioned before, Figure \ref{fig:smartwall1} and Figure \ref{fig:smartwall2} show us a setting of smart wall, where red part is Neumann boundary(opening), and blue part is Dirichlet boundary(wall).

\begin{figure}[ht!]
	\centering
	\includegraphics[scale=0.5]{Images/circle1.eps}
	\caption{A configuration of smart wall in Setting (i)}
	\label{fig:smartwall1}
\end{figure}
\begin{figure}[ht!]
	\centering
	\includegraphics[scale=0.5]{Images/circle2.eps}
	\caption{A configuration of smart wall in Setting (ii)}
	\label{fig:smartwall2}
\end{figure}
\fi

Our goal is to maximize $|u_{x_S}^{k,\epsilon}|^2$, i.e. the norm of Green function at receiver. In numerical implementation, we plot a graph with $\theta$ from $0$ to $2\pi$ as x-axis and $y(\theta):=Re(-\pi\epsilon^3\partial_{\nu_x}G_\Omega^k\left(x_S,\begin{pmatrix}
0 \\ 1
\end{pmatrix}\right)\partial_{\nu_y}G_\Omega^k\left(x_R,\begin{pmatrix}
0 \\ 1
\end{pmatrix}\right))$ as y-axis. Notice that there is infinite sum in $\partial_{\nu_x}G_\Omega^k\left(x_S,\begin{pmatrix}
	0 \\ 1
\end{pmatrix}\right)$ and $\partial_{\nu_y}G_\Omega^k\left(x_R,\begin{pmatrix}
0 \\ 1
\end{pmatrix}\right)$, and we could truncate the sum in \eqref{eq:greenderivative} between $n=-100$ and $n=100$ since all summand outside this range are negligible. Recall we denote $\theta$ as the angle from x-axis to source, and $\tilde{\theta}$ as the angle from x-axis to receiver. Set wave number to be $k=200$, distance between source and origin to be $\rho=0.4$, distance between receiver and origin to be $\tilde\rho = 0.2$, angle difference from receiver to source to be $\pi/3$. We evenly partition the whole boundary into $N=10000$ parts, and empirically set $N/1000=10$ parts left and right of each local maximal point of $y(\theta)$ to be Neumann part. Figure \ref{fig:ploty} shows us the $\theta$-$y(\theta)$ graph, and Figure \ref{fig:smartwall} gives us the corresponding configuration of boundary, with red part as Neumann boundary, and blue part as Dirichlet boundary. The implementation showed us that, the norm of Green function $G_\Omega^k$ with Dirichlet boundary at $x_R$ is 0.067875, while the norm of Green function $u_{x_S}^{k,\epsilon}$ with modified boundary at $x_R$ is 0.790420.

\begin{figure}[ht!]
	\centering
	\includegraphics[scale=0.8]{Images/plot.pdf}
	\caption{Plot of $\theta$-$y(\theta)$}
	\label{fig:ploty}
\end{figure}
\begin{figure}[ht!]
	\centering
	\includegraphics[scale=0.5]{Images/configuration.pdf}
	\caption{A configuration of smart wall}
	\label{fig:smartwall}
\end{figure}
